Boosting Standard Classification Architectures Through a Ranking Regularizer

We employ triplet loss as a feature embedding regularizer to boost classification performance. Standard architectures, like ResNet and Inception, are extended to support both losses with minimal hyper-parameter tuning. This promotes generality while fine-tuning pretrained networks. Triplet loss is a powerful surrogate for recently proposed embedding regularizers. Yet, it is avoided due to large batch-size requirement and high computational cost. Through our experiments, we re-assess these assumptions. During inference, our network supports both classification and embedding tasks without any computational overhead. Quantitative evaluation highlights a steady improvement on five fine-grained recognition datasets. Further evaluation on an imbalanced video dataset achieves significant improvement. Triplet loss brings feature embedding characteristics like nearest neighbor to classification models. Code available at \url{http://bit.ly/2LNYEqL}.

==> honda_exp.tex <==
\section{Experiments}


\subsection{Honda Driving Dataset}
To further demonstrate the softmax plus triplet loss competence, it is evaluated on Honda driving dataset (HDD) ~\cite{RamanishkaCVPR2018} for action recognition. HDD is an realistic ego-motion video dataset for driver behavior understanding and causal reasoning. It contains 10833 valid events spanning ten event classes. The HDD event class distribution is long-tail which poses an imbalanced data challenge. Figure ~\ref{fig:HDD_dist} presents the ten event classes and their distribution. To reduce size and redundancy, video frames are sampled at 3 Hz (three frames per second), events smaller than 2 seconds are considered invalid.\hl{Not sure to present it as 11 event class including background or 10 event classes without background}

To leverage standard architecture for action recognition, Fernando et al.~\cite{fernando2017self} stack of difference (SOD) motion encoding is adapted. While better motion encoding like optical-flow exists, the SOD is utilized for its simplicity and ability to achieve competitive results. Given a sequence of frames representing an event, six consecutive frames spanning 2 seconds are randomly sampled. The six frames are converted to grayscale then every consecutive pair are subtracted as shown in figure ~\ref{fig:sod} to create a stack of difference $\in Z^{W\times H\times 5}$. Standard architectures easily cope with such dimensionality by treating the SOD as a five-channel images instead of three. 

In this experiments, a ResNet50 ~\cite{he2016deep} architecture initialized with random weights and 11-way final softmax layer is employed. It is trained for 10K iterations with a linear decay of the learning rate from an initial value of 0.01, and hyper-parameter  $\lambda=1$. A batch-size of size 33, divisible by 3, is used for fair comparison between the softmax and our proposed approach. All experiments are executed on Titan-Xp $12$GB GPU. To highlight performance on small classes, both micro and macro average accuracies are reported in table ~\ref{tbl:honda_acc}. Macro-average computes the metric independently for each class and then takes the average.
\begin{figure}
	\begin{tikzpicture} \begin{axis}[ ybar,width=0.5\textwidth, height=4.5cm, enlargelimits=0.15, symbolic x coords={Intersection Pass,Left Turn,Right Turn,Left Lane Change,Right Lane Change,Cross-walk passing,U-Turn,Left Lane Branch,Right Lane Branch,Merge}, xtick=data, nodes near coords align={vertical}, x tick label style={rotate=45,anchor=east},] \addplot coordinates {(Intersection Pass,6396) (Left Turn,1673) (Right Turn,1668) (Left Lane Change,600) (Right Lane Change,558) (Cross-walk passing,835) (U-Turn,85) (Left Lane Branch,283) (Right Lane Branch,112) (Merge,172)};  \end{axis}
	\end{tikzpicture}
	\caption{Honda driving dataset long tail class distribution}
	\label{fig:HDD_dist}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=1.0\linewidth]{figures/sod}
	\caption{Motion Encoding using stack of difference. The top row shows a stack of five difference frames constructed by subtracting consecutive pairs of grayscale frames in the bottom row.}
	\label{fig:sod}
\end{figure}

\begin{table}[]
	\begin{tabular}{|l|l|l|}
		\hline
		& Micro Accuracy & Macro  Accuracy \\ \hline
		Vanilla         & 83.73    & 46.09                      \\ \hline
		Hard Batch      &          &                            \\ \hline
		Semi-Hard Batch & 84.55    & 51.20                      \\ \hline
	\end{tabular}
\caption{Quantitative evaluation for action recognition on Honda Dataset. Macro average accuracy is reported to highlight performance on minority event classes.}
\label{tbl:honda_acc}
\end{table}


